Approximated Doubly Robust Search Relevance Estimation

Extracting query-document relevance from the sparse, biased clickthrough log is among the most fundamental tasks in the web search system. Prior art mainly learns a relevance judgment model with semantic features of the query and document and ignores directly counterfactual relevance evaluation from the clicking log. Though the learned semantic matching models can provide relevance signals for tail queries as long as the semantic feature is available. However, such a paradigm lacks the capability to introspectively adjust the biased relevance estimation whenever it conflicts with massive implicit user feedback. The counterfactual evaluation methods, on the contrary, ensure unbiased relevance estimation with sufficient click information. However, they suffer from the sparse or even missing clicks caused by the long-tailed query distribution. In this paper, we propose to unify the counterfactual evaluating and learning approaches for unbiased relevance estimation on search queries with various popularities. Specifically, we theoretically develop a doubly robust estimator with low bias and variance, which intentionally combines the benefits of existing relevance evaluating and learning approaches. We further instantiate the proposed unbiased relevance estimation framework in Baidu search, with comprehensive practical solutions designed regarding the data pipeline for click behavior tracking and online relevance estimation with an approximated deep neural network. Finally, we present extensive empirical evaluations to verify the effectiveness of our proposed framework, finding that it is robust in practice and manages to improve online ranking performance substantially.

==> b_2_related_work.tex <==
\section{Related Work}
We summarize the related literature on {\it Counterfactual Learning to Rank} and {\it Counterfactual Relevance Evaluation} as follows.

\paragraph{Counterfactual Learning to Rank}
The idea of counterfactual learning is to remove the effect of click bias in the computation of local ranking loss so that the model trained with biased data would converge to those trained with unbiased labels. Inverse propensity weighting~(IPW) is a dominant method, which reweights the ranking loss with an inverse propensity score. Early attempts estimate the propensity score by result randomization~\cite{DBLP:conf/wsdm/JoachimsSS17,DBLP:conf/sigir/WangBMN16}. Recent efforts jointly model the 

estimation and unbiased learning to rank. For instance, \citet{DBLP:conf/sigir/AiBLGC18} and \citet{DBLP:conf/www/HuWPL19} present dual learning frameworks for estimating bias and training a ranking model. Further work has extended IPW to various biases, such as trust bias~\cite{10.1145/3308558.3313697}, context bias~\cite{wu2021unbiased}. The other school derives from direct bias modeling methods, which focus on modeling bias factors into click models and extracting true relevance from click signals \cite{DBLP:conf/www/ChapelleZ09, DBLP:conf/wsdm/CraswellZTR08, DBLP:conf/sigir/DupretP08, DBLP:conf/sigir/XuMC10}. For example, \citet{DBLP:conf/recsys/GuoYLTZ19} propose a position-bias aware learning framework for CTR prediction that models position-bias in offline training and conducts online inference without biased information. \citet{DBLP:conf/wsdm/WangGBMN18} unify the training of the ranker model and the estimation of examination propensity with a graphic model and an EM algorithm. \citet{DBLP:conf/www/ZhuangQWBQHC21} study position bias in the grid view and develop cross-positional attention to debias click data.

With the learned generalizable model~(e.g., Match Matrix~\cite{10.5555/3016100.3016292}, Pyramid-ERNIE~\cite{10.1145/3447548.3467147}), counterfactual learning methods are capable of providing relevance estimation, even for those queries with sparse or even missing clicks when the text of query and document is available. However, solely relying on the model might lead to sub-optimal results, since it inherently can not adjust the search results using only the text of query and document, despite the fact that massive user behavioral data can be leveraged to de-bias search results effectively.

\paragraph{Counterfactual Evaluation Methods}
Counterfactual evaluation methods attempt to remove click bias and directly extract the query-document relevance from the clickthrough log. Similar tasks, such as off-policy evaluation~\cite{DBLP:conf/icml/JiangL16,DBLP:conf/icml/DudikLL11}, offline A/B testing~\cite{gilotte2018offline,li2011unbiased}, have been widely studied in reinforcement learning and recommendation. The IPW-based counterfactual learning methods can be applied to counterfactual evaluation by replacing the ranking loss with implicit user feedback. For instance, ~\citet{oosterhuis2020taking} propose the IPW-based estimator for online evaluation. ~\citet{li2015counterfactual} propose to reweight the historical log for policy-evaluation. Furthermore, except for the click behaviors, the after examination behaviors have been explored for interpreting the intrinsic relevance from the clickthrough logs~\cite{dupret2010model}.

With sufficient click information, the evaluation methods can debias user feedback effectively. However, it easily suffers from the sparse or missing clicks caused by the long-tailed query distribution. To make up for the deficiencies of learning and evaluation methods, this work analyzes the properties of each fundamental relevance estimator and devises a novel way to intentionally combine their strengths, yielding a doubly robust relevance estimation framework.

% Model-based methods aim to construct a predictive user model and ask the question of the form "what will the user click if the search result page is presented differently?", which naturally fits debiasing. There are mainly two  directions for the research: (1) knowledge distillation with unbiased data; (2) causal models with biased data.  
% In knowledge distillation, a collection of unbiased data is needed, and it is used to generate unbiased prediction from biased click data. For example, \citet{DBLP:conf/recsys/LinLP021} propose joint reconstruction for knowledge transfer between the biased and unbiased data. 
% In the causal model framework, one needs to design a causal diagram and utilize it to mitigate bias. For instance, ~\citet{DBLP:conf/recsys/LiuCZDHP021} propose a debiased information bottleneck to obtain a debiased representation.
% In general, the work that has the most relevance to ours is~\cite{DBLP:conf/sigir/LiuCDHP020}. This work utilizes knowledge distillation to alleviate bias problem by leveraging uniform data more effectively. However, their work still relies on online result randomization,  and the distilled knowledge need to be re-estimated whenever there are changes in user behaviors. Different from that, our work generates randomization-based data by learning user simulator offline for training a bias-invariant ranker model. 

% ******************* %
% Leveraging implicit user interaction data such as clicks has been shown to be quite encouraging in improving search quality.
% By adopting the user click and non-click feedback as relevance judgment of results, one can simply use this behavioral data for evaluation or training ranking system in the LTR setting.
% However, such naive approach is prone to lead sub-optimal results due to various types of bias in click data, e.g., position bias~\citehere{} and trust bias~\citehere{}.
% In the past, a large amount of research has been devoted to extracting more accurate signals from click data.
% For example, xxx propose xxx, xxx attempt to xxx.
% Nonetheless, despite their effectiveness, these models usually requires that the same query-document pair appears multiple times for reliable inference, making them behave badly for tail queries.



